Sparse spectral methods for partial differential equations on spherical caps

In recent years, sparse spectral methods for solving partial differential equations have been derived using hierarchies of classical orthogonal polynomials on intervals, disks, disk-slices and triangles. In this work we extend the methodology to a hierarchy of non-classical multivariate orthogonal polynomials on spherical caps. The entries of discretisations of partial differential operators can be effectively computed using formulae in terms of (non-classical) univariate orthogonal polynomials. We demonstrate the results on partial differential equations involving the spherical Laplacian and biharmonic operators, showing spectral convergence.

==> spherical-caps copy/bsmacros.tex <==

\usepackage[margin=10pt,font=footnotesize,labelfont=bf]{caption}
\usepackage{subcaption}
\usepackage{float}
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{bm}
\usepackage{bbm}
\usepackage{mleftright}
\usepackage{todonotes}
\usepackage{csquotes}


\newcommand{\sotodo}{\todo[color=green]}
\newcommand{\sotodoinline}{\todo[color=green,inline=true]}
\newcommand{\bstodo}{\todo[color=pink]}
\newcommand{\bstodoinline}{\todo[color=pink,inline=true]}


\usepackage[square,numbers]{natbib}
\usepackage{url}
%\bibliographystyle{elsarticle-harv}
\bibliographystyle{plain}



\usepackage{amsthm}

\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma} 
\newtheorem{theorem}{Theorem} 
\newtheorem{definition}{Definition}
\newtheorem{condition}{Condition}
\newtheorem{algorithm}{Algorithm}
\newtheorem{corollary}{Corollary}
%\newtheorem*{remark}{Remark}
\def\remark{\noindent{\bf Remark}: }

\def\condref#1{Condition~\ref{cond:#1}}

\def\bseqn#1{\begin{align*} #1 \end{align*}}
\def\bseqnnumber#1{\begin{align} #1 \end{align}}
\def\bsset#1#2{\{ #1 \quad | \quad #2 \}}
\def\bsrefeqn#1{equation (\ref{#1})}
\def\bsrefeqns#1#2{equations (\ref{#1}--\ref{#2})}
\def\bsrefsection#1{Section \ref{#1}}
\def\bsreflemma#1{Lemma \ref{#1}}
\def\bsreftheorem#1{Theorem \ref{#1}}
\def\bsrefcor#1{Corollary \ref{#1}}
\def\bsrefdef#1{Definition \ref{#1}}
\def\bsreffig#1{Figure \ref{#1}}




==> spherical-caps copy/bsthesisnewcommands.tex <==
% Thesis/PhD newcommands

%%%%%%
% General
\newcommand{\bigO}{\mathcal{O}}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\No}{\mathbb{N}_0}
\renewcommand{\vec}[1]{\bm{#1}}
\newcommand{\unitvec}[1]{\hat{\bm{#1}}}
\newcommand{\ddx}[1]{{{\rm d} \over {\rm d} #1}}
\newcommand{\ppx}[1]{{\partial \over \partial #1}}
\newcommand{\pfpx}[2]{{\partial #2 \over \partial #1}}
\newcommand{\pmpxm}[2]{{\partial^{#2} \over \partial {#1}^{#2}}}
\newcommand{\dmdxm}[2]{{{\rm d}^{#2} \over {\rm d} {#1}^{#2}}}
\newcommand{\costheta}{\cos\theta}
\newcommand{\sintheta}{\sin\theta}
\newcommand{\cosphi}{\cos\varphi}
\newcommand{\sinphi}{\sin\varphi}
\newcommand{\eimphi}{e^{im\varphi}}
\newcommand{\eimtheta}{e^{im\theta}}
\newcommand{\phivec}{\hat{\bm{\phi}}}
\newcommand{\thetavec}{\hat{\bm{\theta}}}


\newcommand{\mtrx}[1]{#1}
\newcommand{\idmat}[1]{\mtrx{I}_{#1}}
\newcommand{\zeromat}[1]{\mtrx{0}_{#1}}

\newcommand{\divergence}{\nabla \cdot}
\newcommand{\grad}{\nabla}
\newcommand{\DeltaS}{\Delta_{\rm S}}
\newcommand{\gradS}{\nabla_{\rm S}}

% fancy letters
\newcommand{\calA}{\mathcal{A}}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calE}{\mathcal{E}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\bigP}{\mathbb{P}}
\newcommand{\bigT}{\mathbb{T}}



%%%%%%
% Thesis specific

% SH
\newcommand{\Ylm}{Y^m_l}
\newcommand{\Ylmfull}{Y^m_l(\theta,\varphi)}
\newcommand{\Plm}{\jac^m_l}
\newcommand{\alphalm}{\alpha^m_l}
\newcommand{\clm}{c^m_l}
\newcommand{\ctilde}{\tilde{c}^m_l}
\newcommand{\ctildemod}{\tilde{c}^{|m|}_l}
\newcommand{\chat}{\hat{c}^m_l}
\newcommand{\chatmod}{\hat{c}^{|m|}_l}
%\newcommand{\ddx}{\frac{\mathrm{d}}{\mathrm{d}x}}
%\newcommand{\ddy}{\frac{\mathrm{d}}{\mathrm{d}y}}
%\newcommand{\pddx}{\frac{\partial}{\partial x}}
%\newcommand{\pddy}{\frac{\partial}{\partial y}}
%\newcommand{\pddn}{\frac{\partial}{\partial n}}
%\newcommand{\dmdxm}{\frac{\mathrm{d}^m}{\mathrm{d}x^m}}

\newcommand{\Atilde}{\tilde{A}_{l,m}}
\newcommand{\Btilde}{\tilde{B}_{l,m}}
\newcommand{\Dtilde}{\tilde{D}_{l,m}}
\newcommand{\Etilde}{\tilde{E}_{l,m}}
\newcommand{\Ftilde}{\tilde{F}_{l,m}}
\newcommand{\Gtilde}{\tilde{G}_{l,m}}
\newcommand{\Alm}{A_{l,m}}
\newcommand{\Blm}{B_{l,m}}
\newcommand{\Dlm}{D_{l,m}}
\newcommand{\Elm}{E_{l,m}}
\newcommand{\Flm}{F_{l,m}}
\newcommand{\Glm}{G_{l,m}}

\newcommand{\xione}{\xi^{(1)}_{n, \lambda}}
\newcommand{\xitwo}{\xi^{(2)}_{n, \lambda}}
\newcommand{\xithree}{\xi^{(3)}_{n, \lambda}}
\newcommand{\xifour}{\xi^{(4)}_{n, \lambda}}


\newcommand{\SHvec}{\bigP}
\newcommand{\SHvecl}{\SHvec_l}
\newcommand{\VSHvec}{\bigT}
\newcommand{\VSHvecperp}{\VSHvec^\perp}
\newcommand{\VSHvecfull}{\tilde{\bigT}}
\newcommand{\VSHvecl}{\VSHvec_l}
\newcommand{\VSHvecperpl}{\VSHvecperp_l}
\newcommand{\VSHvecfulll}{\VSHvecfull_l}
\newcommand{\gradY}{\nabla Y}
\newcommand{\gradYlm}{\nabla Y^m_l}
\newcommand{\gradpY}{\nabla^\perp Y}
\newcommand{\gradpYlm}{\nabla^\perp Y^m_l}

\newcommand{\Dlt}{D^\top_l}

\newcommand{\curlyy}{\bm{\mathcal{Y}}}
\newcommand{\blone}{\beta_{l, 1}}
\newcommand{\blzero}{\beta_{l, 0}}
\newcommand{\blmone}{\beta_{l, -1}}
\newcommand{\chivec}{\bm{\chi}_{1,m_s}}
\newcommand{\cgcoeff}{\mathcal{C}}

\newcommand{\alm}{a_{l,m}}
\newcommand{\blm}{b_{l,m}}
\newcommand{\dlm}{d_{l,m}}
\newcommand{\elm}{e_{l,m}}
\newcommand{\flm}{f_{l,m}}
\newcommand{\glm}{g_{l,m}}
\newcommand{\hlm}{h_{l,m}}
\newcommand{\jlm}{j_{l,m}}
\newcommand{\klm}{k_{l,m}}
\newcommand{\almperp}{a_{l,m}^\perp}
\newcommand{\blmperp}{b_{l,m}^\perp}
\newcommand{\dlmperp}{d_{l,m}^\perp}
\newcommand{\elmperp}{e_{l,m}^\perp}
\newcommand{\flmperp}{f_{l,m}^\perp}
\newcommand{\glmperp}{g_{l,m}^\perp}
\newcommand{\hlmperp}{h_{l,m}^\perp}
\newcommand{\jlmperp}{j_{l,m}^\perp}
\newcommand{\klmperp}{k_{l,m}^\perp}



% Disk-Slice
\newcommand{\hdop}{H}
\newcommand{\bighdop}{\mathbb{\hdop}}
\newcommand{\hdopnk}{\hdop_{n,k}}
\newcommand{\hdopnkab}{\hdop_{n,k}^{(a,b)}}
\newcommand{\hdopab}{\hdop^{(a,b)}}
\newcommand{\Wab}{{W^{(a,b)}}}
\newcommand{\hdopmj}{\hdop_{m,j}}
\newcommand{\hdopmjab}{\hdop_{m,j}^{(a,b)}}
\newcommand{\alphaab}{\alpha^{(a,b)}}
\newcommand{\betaab}{\beta^{(a,b)}}
\newcommand{\bighdopab}{\bighdop^{(a,b)}}
\newcommand{\Dnt}{D^\top_n}
\newcommand{\Wii}{W^{(1,1)}}
\newcommand{\hdopii}{\hdop^{(1,1)}}
\newcommand{\bighdopii}{{\mathbb{\hdop}^{(1,1)}}}
\newcommand{\hdopoo}{\hdop^{(0,0)}}
\newcommand{\bighdopoo}{{\mathbb{\hdop}^{(0,0)}}}
\newcommand{\hdopoi}{\hdop^{(0,1)}}
\newcommand{\hdopio}{\hdop^{(1,0)}}
%\newcommand{\jac}{{\tilde P}}
\newcommand{\jac}{{P}}
\newcommand{\genjac}{R}
\newcommand{\genjacnmk}{\genjac_{n-k}}
\newcommand{\genjacmmj}{\genjac_{m-j}}
\newcommand{\genjacw}{w_\genjac}
\newcommand{\jacw}{w_P}
\newcommand{\normgenjac}{\omega_\genjac}
\newcommand{\normjac}{\omega_P}

%\newcommand{\dx}{\frac{\partial}{\partial x}}
%\newcommand{\dy}{\frac{\partial}{\partial y}}
\newcommand{\laplacewii}{\Delta_W^{(1,1)\to(1,1)}}
\newcommand{\laplacewtt}{\Delta_W^{(2,2)\to(0,0)}}
\newcommand{\laplaceoo}{\Delta^{(0,0)\to(2,2)}}
\newcommand{\biharmonic}{_2\Delta_W^{(2,2)\to(2,2)}}

\newcommand{\element}{\tau}
\newcommand{\refelement}{\hat{\tau}}
\newcommand{\FEset}{\mathcal{T}}
\newcommand{\bigW}{\mathbb{W}}
\newcommand{\bigWab}{\mathbb{W}^{(a,b)}}
\newcommand{\bigWii}{{\mathbb{W}^{(1,1)}}}
\newcommand{\bigQ}{\mathbb{Q}}
\newcommand{\bigQab}{\bigQ^{(a,b)}}


\newcommand{\hdopnkabc}{\hdop_{n,k}^{(a,b,c)}}
\newcommand{\hdopabc}{\hdop^{(a,b,c)}}
\newcommand{\Wabc}{{W^{(a,b,c)}}}
\newcommand{\hdopmjabc}{\hdop_{m,j}^{(a,b,c)}}
\newcommand{\alphaabc}{\alpha^{(a,b,c)}}
\newcommand{\betaabc}{\beta^{(a,b,c)}}
\newcommand{\bighdopabc}{\bighdop^{(a,b,c)}}
\newcommand{\Wiii}{W^{(1,1,1)}}
\newcommand{\hdopiii}{\hdop^{(1,1,1)}}
\newcommand{\bighdopiii}{{\mathbb{\hdop}^{(1,1,1)}}}
\newcommand{\hdopooo}{\hdop^{(0,0,0)}}
\newcommand{\bighdopooo}{{\mathbb{\hdop}^{(0,0,0)}}}
\newcommand{\hdopooi}{\hdop^{(0,0,1)}}
\newcommand{\hdopiio}{\hdop^{(1,1,0)}}
\newcommand{\laplacewiii}{\Delta_W^{(1,1,1)\to(1,1,1)}}
\newcommand{\laplacewttt}{\Delta_W^{(2,2,2)\to(0,0,0)}}
\newcommand{\laplaceooo}{\Delta^{(0,0,0)\to(2,2,2)}}
\newcommand{\biharmonictwo}{_2\Delta_W^{(2,2,2)\to(2,2,2)}}
\newcommand{\bigWiii}{{\mathbb{W}^{(1,1,1)}}}
\newcommand{\bigWabc}{\mathbb{W}^{(a,b,c)}}

\newcommand{\alphaabcd}{\alpha^{(a,b,c,d)}}
\newcommand{\betaabcd}{\beta^{(a,b,c,d)}}
\newcommand{\hdopnkabcd}{\hdop_{n,k}^{(a,b,c,d)}}
\newcommand{\hdopabcd}{\hdop^{(a,b,c,d)}}
\newcommand{\Wabcd}{{W^{(a,b,c,d)}}}
\newcommand{\hdopmjabcd}{\hdop_{m,j}^{(a,b,c,d)}}
\newcommand{\bighdopabcd}{\bighdop^{(a,b,c,d)}}
\newcommand{\bigWabcd}{\mathbb{W}^{(a,b,c,d)}}

\newcommand{\genjact}{\tilde{\genjac}}
\newcommand{\genjactnmk}{\genjact_{n-k}}
\newcommand{\genjactmmj}{\genjact_{m-j}}
\newcommand{\genjactw}{w_{\genjact}}
\newcommand{\normgenjact}{\omega_{\genjact}}


% Spherical Cap
\newcommand{\scop}{Q}
\newcommand{\scopnki}{\scop_{n,k,i}}
\newcommand{\scopmjh}{\scop_{m,j,h}}
\newcommand{\scopa}{\scop^{(a)}}
\newcommand{\scopnkia}{\scopnki^{(a)}}
\newcommand{\scopmjha}{\scopmjh^{(a)}}
\newcommand{\bigscop}{{\mathbb{\tilde Q}}}
\newcommand{\bigscopa}{\bigscop^{(a)}}
\newcommand{\bigscopN}{\bigscop_{N}}
\newcommand{\bigscopNa}{\bigscopa_{N}}
\newcommand{\bigscopNka}{\bigscopa_{N,k}}
\newcommand{\bigscopt}{\mathbb{{Q}}}
\newcommand{\bigscopta}{\bigscopt^{(a)}}
\newcommand{\bigscoptn}{\bigscopt_{n}}
\newcommand{\bigscoptna}{\bigscopta_{n}}
\newcommand{\xvec}{\mathbf{x}}
\newcommand{\ch}{Y}
\newcommand{\chki}{\ch_{k,i}}
\newcommand{\chjh}{\ch_{j,h}}
\newcommand{\chkitheta}{\ch_{k,i}(\theta)}
\newcommand{\alphaa}{\alpha^{(a)}}
\newcommand{\betaa}{\beta^{(a)}}
\newcommand{\gammaa}{\gamma^{(a)}}
\newcommand{\Wa}{W^{(a)}}
\newcommand{\bigWNa}{\mathbb{W}_N^{(a)}}
\newcommand{\ddz}{\ddx{z}}
\newcommand{\ppz}{\ppx{z}}
\newcommand{\ppphi}{\ppx{\varphi}}
\newcommand{\rhoppphi}{\rho \ppphi}
\newcommand{\rhozppphi}{\rho(z) \ppphi}
\newcommand{\pptheta}{\ppx{\theta}}
\newcommand{\ppthetatwo}{{\partial^2 \over \partial \theta^2}}
\newcommand{\bigWNi}{\mathbb{W}_N^{(1)}}
\newcommand{\scopi}{\scop^{(1)}}
\newcommand{\scopnkii}{\scopnki^{(1)}}
\newcommand{\bigWNo}{\mathbb{W}_N^{(0)}}
\newcommand{\scopo}{\scop^{(0)}}
\newcommand{\scopnkio}{\scopnki^{(0)}}
\newcommand{\bigscopi}{\bigscop^{(1)}}
\newcommand{\bigscopNi}{\bigscopi_{N}}
\newcommand{\bigscopNki}{\bigscopi_{N,k}}
\newcommand{\bigscopo}{\bigscop^{(0)}}
\newcommand{\bigscopNo}{\bigscopo_{N}}
\newcommand{\bigscopNko}{\bigscopo_{N,k}}


% Tangent space
\newcommand{\tangentspace}{{\Omega_T}}
\newcommand{\bigtsop}{\mathbb{T}}
\newcommand{\bigtsopt}{\tilde{\bigtsop}}
\newcommand{\bigtsoptn}{\bigtsopt_n}
\newcommand{\bigtsopN}{\bigtsop_N}
\newcommand{\bigtsopNk}{\bigtsop_{N,k}}
\newcommand{\tsopi}{\bm{\Phi}}
\newcommand{\tsopii}{\bm{\Psi}}
\newcommand{\tsopiN}{\tsopi_N}
\newcommand{\tsopiiN}{\tsopii_N}
\newcommand{\tsopinki}{\tsopi_{n,k,i}}
\newcommand{\tsopiinki}{\tsopii_{n,k,i}}
\newcommand{\tsopinkit}{\tsopi_{n,k,i}^\top}
\newcommand{\tsopiinkit}{\tsopii_{n,k,i}\top}
\newcommand{\tsopit}{\tsopi^\top}
\newcommand{\tsopiit}{\tsopii^\top}
\newcommand{\rvec}{\hat{\bm{r}}}
\newcommand{\jacobimattangent}{{}^T\!J}
\newcommand{\jacobimattangentx}{\jacobimattangent_x}
\newcommand{\jacobimattangenty}{\jacobimattangent_y}
\newcommand{\jacobimattangentz}{\jacobimattangent_z}
\newcommand{\alphao}{\alpha^{(0)}}
\newcommand{\alphaonkj}{\alphao_{n,k,j}}
\newcommand{\betao}{\beta^{(0)}}
\newcommand{\betaonkj}{\betao_{n,k,j}}
\newcommand{\gammao}{\gamma^{(0)}}
\newcommand{\gammaonkj}{\gammao_{n,k,j}}
\newcommand{\uvec}{\bm{u}}
\newcommand{\fvec}{\bm{f}}
\newcommand{\hvec}{\bm{h}}
\newcommand{\uvecc}{\uvec^c}
\newcommand{\fvecc}{\fvec^c}
\newcommand{\hvecc}{\hvec^c}
\newcommand{\uvecn}{\uvec_n}
\newcommand{\hvecn}{\hvec_n}
\newcommand{\uvecnpi}{\uvec_{n+1}}
\newcommand{\hvecnpi}{\hvec_{n+1}}
\newcommand{\uvecnc}{\uvecc_n}
\newcommand{\hvecnc}{\hvecc_n}
\newcommand{\uvecnpic}{\uvecnpi^c}
\newcommand{\hvecnpic}{\hvecnpi^c}
\newcommand{\href}{\mathcal{H}}
\newcommand{\tangentjacobi}{{}^T\!J}
\newcommand{\uveccperp}{\uvec^{\perp c}}
\newcommand{\uvecncperp}{\uveccperp_n}






==> spherical-caps copy/somacros.tex <==

\def\addtab#1={#1\;&=}

\def\meeq#1{\def\ccr{\\\addtab}
%\tabskip=\@centering
 \begin{align*}
 \addtab#1
 \end{align*}
  }  
  
  \def\leqaddtab#1\leq{#1\;&\leq}
  \def\mleeq#1{\def\ccr{\\\addtab}
%\tabskip=\@centering
 \begin{align*}
 \leqaddtab#1
 \end{align*}
  }  


\def\vc#1{\mbox{\boldmath$#1$\unboldmath}}

\def\vcsmall#1{\mbox{\boldmath$\scriptstyle #1$\unboldmath}}

\def\vczero{{\mathbf 0}}


%\def\beginlist{\begin{itemize}}
%
%\def\endlist{\end{itemize}}


\def\pr(#1){\left({#1}\right)}
\def\br[#1]{\left[{#1}\right]}
\def\fbr[#1]{\!\left[{#1}\right]}
\def\set#1{\left\{{#1}\right\}}
\def\ip<#1>{\left\langle{#1}\right\rangle}
\def\iip<#1>{\left\langle\!\langle{#1}\right\rangle\!\rangle}

\def\norm#1{\left\| #1 \right\|}

\def\abs#1{\left|{#1}\right|}
\def\fpr(#1){\!\pr({#1})}

\def\Re{{\rm Re}\,}
\def\Im{{\rm Im}\,}

\def\floor#1{\left\lfloor#1\right\rfloor}
\def\ceil#1{\left\lceil#1\right\rceil}


\def\mapengine#1,#2.{\mapfunction{#1}\ifx\void#2\else\mapengine #2.\fi }

\def\map[#1]{\mapengine #1,\void.}

\def\mapenginesep_#1#2,#3.{\mapfunction{#2}\ifx\void#3\else#1\mapengine #3.\fi }

\def\mapsep_#1[#2]{\mapenginesep_{#1}#2,\void.}


\def\vcbr[#1]{\pr(#1)}


\def\bvect[#1,#2]{
{
\def\dots{\cdots}
\def\mapfunction##1{\ | \  ##1}
	\sopmatrix{
		 \,#1\map[#2]\,
	}
}
}

\def\vect[#1]{
{\def\dots{\ldots}
	\vcbr[{#1}]
}}

\def\vectt[#1]{
{\def\dots{\ldots}
	\vect[{#1}]^{\top}
}}

\def\Vectt[#1]{
{
\def\mapfunction##1{##1 \cr} 
\def\dots{\vdots}
	\begin{pmatrix}
		\map[#1]
	\end{pmatrix}
}}



\def\thetaB{\mbox{\boldmath$\theta$}}
\def\zetaB{\mbox{\boldmath$\zeta$}}


\def\newterm#1{{\it #1}\index{#1}}


\def\TT{{\mathbb T}}
\def\C{{\mathbb C}}
\def\R{{\mathbb R}}
\def\II{{\mathbb I}}
\def\F{{\mathcal F}}
\def\E{{\rm e}}
\def\I{{\rm i}}
\def\D{{\rm d}}
\def\dx{\D x}
\def\dy{\D y}
\def\CC{{\cal C}}
\def\DD{{\cal D}}
\def\U{{\mathbb U}}
\def\A{{\cal A}}
\def\K{{\cal K}}
\def\DTU{{\cal D}_{{\rm T} \rightarrow {\rm U}}}
\def\LL{{\cal L}}
\def\B{{\cal B}}
\def\T{{\cal T}}
\def\W{{\cal W}}


\def\tF_#1{{\tt F}_{#1}}
\def\Fm{\tF_m}
\def\Fab{\tF_{\alpha,\beta}}
\def\FC{\T}
\def\FCpmz{\FC^{\pm {\rm z}}}
\def\FCz{\FC^{\rm z}}

\def\tFC_#1{{\tt T}_{#1}}
\def\FCn{\tFC_n}

\def\rmz{{\rm z}}

\def\chapref#1{Chapter~\ref{Chapter:#1}}
\def\secref#1{Section~\ref{Section:#1}}
\def\exref#1{Exercise~\ref{Exercise:#1}}
\def\lmref#1{Lemma~\ref{Lemma:#1}}
\def\propref#1{Proposition~\ref{Proposition:#1}}
\def\warnref#1{Warning~\ref{Warning:#1}}
\def\thref#1{Theorem~\ref{Theorem:#1}}
\def\defref#1{Definition~\ref{Definition:#1}}
\def\probref#1{Problem~\ref{Problem:#1}}
\def\corref#1{Corollary~\ref{Corollary:#1}}
\def\appref#1{Appendix~\ref{Appendix:#1}}

\def\sgn{{\rm sgn}\,}
\def\Ai{{\rm Ai}\,}
\def\Bi{{\rm Bi}\,}
\def\wind{{\rm wind}\,}
\def\erf{{\rm erf}\,}
\def\erfc{{\rm erfc}\,}
\def\qqquad{\qquad\quad}
\def\qqqquad{\qquad\qquad}


\def\spand{\hbox{ and }}
\def\spodd{\hbox{ odd}}
\def\speven{\hbox{ even}}
\def\qand{\quad\hbox{and}\quad}
\def\qqand{\qquad\hbox{and}\qquad}
\def\qfor{\quad\hbox{for}\quad}
\def\qqfor{\qquad\hbox{for}\qquad}
\def\qas{\quad\hbox{as}\quad}
\def\qqas{\qquad\hbox{as}\qquad}
\def\qor{\quad\hbox{or}\quad}
\def\qqor{\qquad\hbox{or}\qquad}
\def\qqwhere{\qquad\hbox{where}\qquad}



%%% Words

\def\naive{na\"\i ve\xspace}
\def\Jmap{Joukowsky map\xspace}
\def\Mobius{M\"obius\xspace}
\def\Holder{H\"older\xspace}
\def\Mathematica{{\sc Mathematica}\xspace}
\def\apriori{apriori\xspace}
\def\WHf{Weiner--Hopf factorization\xspace}
\def\WHfs{Weiner--Hopf factorizations\xspace}

\def\Jup{J_\uparrow^{-1}}
\def\Jdown{J_\downarrow^{-1}}
\def\Jin{J_+^{-1}}
\def\Jout{J_-^{-1}}



\def\bD{\D\!\!\!^-}




\def\questionequals{= \!\!\!\!\!\!{\scriptstyle ? \atop }\,\,\,}

\def\elll#1{\ell^{\lambda,#1}}
\def\elllp{\ell^{\lambda,p}}
\def\elllRp{\ell^{(\lambda,R),p}}


\def\elllRpz_#1{\ell_{#1{\rm z}}^{(\lambda,R),p}}


\def\sopmatrix#1{\begin{pmatrix}#1\end{pmatrix}}

\def\socases#1{\begin{cases} #1 \end{cases}}


\def\Problem#1#2\par{\begin{problem}\label{pb:#1} #2\end{problem}}
\def\Theorem#1#2\par{\begin{theorem}\label{th:#1} #2\end{theorem}}
\def\Conjecture#1#2\par{\begin{conjecture}\label{conj:#1} #2\end{conjecture}}
\def\Proposition#1#2\par{\begin{proposition}\label{prop:#1} #2\end{proposition}}
\def\Definition#1#2\par{\begin{definition}\label{def:#1} #2\end{definition}}
\def\Corollary#1#2\par{\begin{corollary}\label{cr:#1} #2\end{corollary}}
\def\Lemma#1#2\par{\begin{lemma}\label{lm:#1} #2\end{lemma}}
\def\Example#1#2\par{\begin{example}\label{ex:#1} #2\end{example}}
\def\Remark #1\par{\begin{remark*}#1\end{remark*}}


\def\Proof{\begin{proof}}
\def\mqed{\end{proof}}


\def\Figuretwow[#1,#2]#3#4\par{
\begin{figure}[tb]
\begin{center}{
\includegraphics[width=#3]{Figures/#1}\includegraphics[width=#3]{Figures/#2}}
\end{center}
\caption{#4}\label{fig:#1} 
\end{figure}
}
